MithraDetective: A System for Cherry-picked Trendlines Detection

Given a data set, misleading conclusions can be drawn from it by cherry-picking selected samples. One important class of conclusions is a trend derived from a data set of values over time. Our goal is to evaluate whether the 'trends' described by the extracted samples are representative of the true situation represented in the data. We demonstrate MithraDetective, a system to compute a support score to indicate how cherry-picked a statement is; that is, whether the reported trend is well-supported by the data. The system can also be used to discover more supported alternatives. MithraDetective provides an interactive visual interface for both tasks.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

==> architecture.tex <==
% \begin{figure}
%      \centering
%      \includegraphics[width=0.5\textwidth]{figures/Architecture.png}
%      \caption{Architecture of MithraRanking}
%      \label{fig:architecture}
% \end{figure}


\begin{figure*}[t]
 \centering
 \includegraphics[width=.95\textwidth]{figures/User_Interface.png}
 \vspace{-6mm}\caption{\small \mr: User Interface}
 \label{fig:user_interface}
 \vspace{-5mm}
\end{figure*}

\section{System Details}\label{sec:system}
% In this section, we describe the architecture of MithraRanking system and its user interface.

\subsection{Architecture and Implementation}\label{subsec:arch}
    % Fig.~\ref{fig:architecture} shows the architecture of
    MithraRanking is a Web application. % A user connects to it via the Internet and optionally uploads datasets by making HTTP requests.
    The user uploads a dataset, or chooses among available datasets, and specifies fairness criteria and ranking attributes. She then identifies a region of interest (as an initial weight vector and a cosine similarity bound).  %This information is sent to the back-end server, which processes the clients' request, 
    The system then ranks the data based on the specified ranking function and checks if the ranking satisfies the fairness criteria. Then, it draws unbiased function samples (using the method in~\cite{stableranking}) from the region of interest to estimate the stability of the generated ranking. It also uses the samples for finding the most stable rankings in the region of interest, the ``closest'' fair function in the neighborhood of the input function, and a function (not necessarily the closest) that generates a fair and more stable ranking.  The user can then accept any of those suggestions and change the ranking accordingly.
    
    It is possible that no acceptable function is found even after exhausting the sampling budget, either because such a  function does not exist in the specified region, or because the function exists but the sampling did not find it. The system allows the user to (i) try again by taking more samples,
    %and exploring the region of interest further
    (ii) increase the region of interest by reducing the cosine similarity requirement between the input and suggested functions, (iii) change the input function to a different meaningful function, (iv) relax the fairness criteria, or (v) conclude that the dataset is not a good fit for this task. %and %resolve the bias in it, for example by acquiring 
    %acquire more data.

% \subsection{Technical Challenges}\label{subsec:arch}

% \subsection{System Implementation} 
MithraRanking is implemented using {\em Python 2.7.10}. To build the Web service, we used {\em Flask framework}, due to its flexibility and fine-grained control. We used {\em Pandas} and {\em NumPy} libraries to process datasets. On the client side, {\em AngularJS 1.6.9}, {\em Bootstrap 4.0.0}, {\em jQuery}, {\em HTML}, and {\em CSS} are used to parse results from the back-end and to render pages.

% \textcolor{red}{Added technical challenge. Delete it if unnecessary}
% We faced two main technical challenges in practice. First, sampling does not guarantee the discovery of an approximation solution. Currently, we allow users to try many times until our system finds one desirable rankings. This can be computationally expensive in worst cases. In the future, we could provide an option to pre-process users' datasets and notify them by emails when this process is done. This would make users play with our system quicker. Second, our system might have different users playing different datasets at the same time. Thus, sequential processing of datasets and queries may significantly reduce system performance. We applied parallel processing to reduce the wait time of users.



% \begin{figure}
%      \centering
%      \includegraphics[width=0.5\textwidth]{figures/fig2.png}
%      \caption{Steps 2 and 3: Setting up the fairness criteria and ranking region}
%      \label{fig:step2}
% \end{figure}


\subsection{User Interface}\label{subsec:userInterface}
MithraRanking has four main sections in its user interface, which we describe in turn below.
%(i) Dataset Selection section, (ii) Fairness Criteria section , (iii) Ranking section, and (iv) Ranking Results section. 

\noindent
\textbf{Dataset Selection section:} The first thing a user has to do is to specify the dataset of interest. Each tuple in this dataset is an item to be ranked, based on the values of its attributes. As shown in Fig.~\ref{fig:user_interface}(a), users can either select a dataset from our pre-loaded demonstration datasets or upload their own dataset to design their ranking schemes.
% Of course, in actual use, only the latter path will be taken. The former is meant for users who want to play with our system before using it for their actual data.

\noindent\textbf{Fairness Criteria section:} This is the section where users define the fairness criteria.
In line with prior work~\cite{DBLP:conf/kdd/FeldmanFMSV15,StoyanovichYJ18,DBLP:conf/ssdbm/YangS17}, we define fairness with regard to {\em sensitive attributes}, which denote membership of individuals in legally-protected categories, such as people with disabilities, or under-represented minorities by gender or ethnicity.
While our techniques apply to a broad range of fairness criteria~\cite{fairranking}, in our system, we define fairness in terms of minimum/maximum bounds on the number of selected members of a protected group at the top-$k$, for some reasonable value of $k$~\cite{DBLP:conf/icalp/CelisSV18}.
Fig.~\ref{fig:user_interface}(b) shows the fairness criteria section.
The user first should identify the value of $k$ for analyzing fairness (it is 30\% in the figure).
Then the user can add multiple fairness criteria by selecting (a) the direction to be at most/at least, (b) the percentage, (c) a sensitive attribute, (d) the criteria condition (=, $\neq$, $<$, $>$, $\geq$, or $\leq$), and (e) an attribute value.
For instance, in the figure the added fairness criterion is "at most 50\% with age$\geq$ 56 in top 30\%", %meaning that the number of individuals with age more than 56 should at most be 50\% in the top-$k$ (30\% in this figure), 
or the ranking is not fair.

\noindent\textbf{Ranking section:} As demonstrated in Fig.~\ref{fig:user_interface}(c), users can add ranking attributes from drop-down menus and assign weights to them using sliders. If they want to change ranking attributes, they can click the ``remove'' button to delete unnecessary attributes. At the bottom of Fig.~\ref{fig:user_interface}(c), users can specify a value of cosine similarity. This value
defines a {\em ``region of interest''}~\cite{stableranking} around the specified ranking function (weight vector) within which all weights are equally acceptable.
For example, the value 98\% in the figure indicates that all weight vectors that have at least 98\% cosine similarity with the specified weight vector are within the region of interest.
This region is considered for computing the {\em stability} of the produced ranking by specified ranking, and to discover the most stable ranking.
We also use this region for exploration to find a fair function in vicinity of the specified function, in case its output is not fair. 

\noindent\textbf{Ranking Results section:} The ranking results section
provides (a) the ranking generated by the specified function, (b) a signal indicating if the generated ranking is fair and/or stable, and (c) information about the suggested functions. 
The reference ranking is depicted in Fig.~\ref{fig:user_interface}(d), in the form of a table containing tuples ranked based on the user-specified ranking function, with a pagination bar under the table for users to navigate through the table. 
The fairness and stability signals, as well as function suggestions are provided in Fig.~\ref{fig:user_interface}(e).
As shown in the figure, we list three suggestion options to the user:
(i) the closest fair function, (ii) the closest function that generates the most stable ranking, and (iii) a function that is fair (not necessarily the closest) and more stable than the reference function.
There are inherent trade-offs between fairness, stability, and distance from the user's original choice, If the system could not find proper functions, or the user is not satisfied with system's suggestions, she can ``explore more'' by taking more samples from the region of interest (of course the user can also apply changes in prior steps such as input function or region of interest and re-try).



% We list three suggestion options: (i) Fair, (ii) Most Stable, and (iii) Fair and More stable in table format as demonstrated in Fig.~\ref{fig:user_interface}(e). If our system could find such options, there will be accept buttons on the last row of the table. If not, there will be dashes indicating we could not find these options given the limited amount of budget (i.e. the maximum times our system try). If users are satisfied with either one of these three options and our system successfully finds that option, they can click the corresponding accept button to accept suggested weights. However, they can click the explore more button to let our system try more budget if they are not satisfied with the results.



==> cssxml.tex <==

%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below.
%
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10002951.10003317</concept_id>
       <concept_desc>Information systems~Information retrieval</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10002951.10003317.10003359.10011699</concept_id>
       <concept_desc>Information systems~Presentation of retrieval results</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Information systems~Information retrieval}
\ccsdesc[500]{Information systems~Presentation of retrieval results}
